On the Reconstruction of Orthomodular Logic via Restricted Negation

Orthomodular logic has long been studied as a fundamental logical framework within quantum logic. In addition to its lattice-theoretic foundations, various formulations have been proposed that incorporate specialized implication connectives and more complex logical connectives. In this study, we reconstruct orthomodular logic by introducing a connective referred to as restricted negation, which has received comparatively little attention in the existing literature. We demonstrate that this connective provides a natural and expressive basis for formulating the core principles of orthomodular logic. Furthermore, as a main result, we construct a new proof system for orthomodular logic founded on this connective.

==> eptcsdata.tex <==
\providecommand{\firstpage}{47}
\providecommand{\publicationstatus}{A. Indrzejczak, T. Jarmu\.zek, M. Klonowski, \& M. Zawidzki (Eds.):\\ Twelfth International Conference on\\ Non-Classical Logics. Theory and Applications (NCL'26)\\
EPTCS 455, 2026, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.455.5}{10.4204/EPTCS.455.5}}
\pdfoutput=1

